SASMU: boost the performance of generalized recognition model using synthetic face dataset

Nowadays, deploying a robust face recognition product becomes easy with the development of face recognition techniques for decades. Not only profile image verification but also the state-of-the-art method can handle the in-the-wild image almost perfectly. However, the concern of privacy issues raise rapidly since mainstream research results are powered by tons of web-crawled data, which faces the privacy invasion issue. The community tries to escape this predicament completely by training the face recognition model with synthetic data but faces severe domain gap issues, which still need to access real images and identity labels to fine-tune the model. In this paper, we propose SASMU, a simple, novel, and effective method for face recognition using a synthetic dataset. Our proposed method consists of spatial data augmentation (SA) and spectrum mixup (SMU). We first analyze the existing synthetic datasets for developing a face recognition system. Then, we reveal that heavy data augmentation is helpful for boosting performance when using synthetic data. By analyzing the previous frequency mixup studies, we proposed a novel method for domain generalization. Extensive experimental results have demonstrated the effectiveness of SASMU, achieving state-of-the-art performance on several common benchmarks, such as LFW, AgeDB-30, CA-LFW, CFP-FP, and CP-LFW.

==> supplementary_files/SA_ablation_AC_Equalize_prbabilty.tex <==
\subsection{Revisiting grayscale and similar augmentation}
\label{sec:abl_probability}
After selecting the basic appearance and geometry data augmentation, we find that appearance augmentation could efficiently improve the model generalization, leading to better performance in real-world image tests. To explore the potential of appearance augmentation while avoiding the risk of losing facial details, such as adding excessive noise or using GAN-based image editing that requires an additional model, we consider two smooth data augmentations: histogram equalization and autocontrast. As shown in the experiment details listed in Table~\ref{table:equalization_and_autocontrast} and the results in Table~\ref{tab:abl_equalization_and_autocontrast}, both histogram equalization and autocontrast improve the test results, but histogram equalization has a greater impact than autocontrast. To keep the data augmentation list manageable, we decide to use only histogram equalization. In addition, we make an interesting discovery that the experiments of both histogram equalization and autocontrast suggest setting their probability to 1, which is counterintuitive. 
% We further experiment with grayscale to validate this finding and avoid any accidental results.

%SA-B0-Equal0:DataAug32
%SA-B0-Equal1:DataAug33
%SA-B1-Equal1:DataAug34
%SA-B1-Equal2:DataAug35
%SA-B0-Equal3:DataAug37
%SA-B1-Equal3:DataAug36

%SA-B0-AC0:DataAug38
%SA-B0-AC1:DataAug39
%SA-B1-AC1:DataAug40
%SA-B1-AC2:DataAug41
%SA-B0-AC3:DataAug43
%SA-B1-AC3:DataAug42



%SA-B0-Equal0:DataAug32
%SA-B0-Equal1:DataAug33
%SA-B1-Equal1:DataAug34
%SA-B1-Equal2:DataAug35
%SA-B0-Equal3:DataAug37
%SA-B1-Equal3:DataAug36

%SA-B0-AC0:DataAug38
%SA-B0-AC1:DataAug39
%SA-B1-AC1:DataAug40
%SA-B1-AC2:DataAug41
%SA-B0-AC3:DataAug43
%SA-B1-AC3:DataAug42



We further conduct experiments on histogram equalization based on \textbf{SA-B4-Per1} in Section \ref{sec:abl_geometry}, but varied the probability of grayscale, as shown in Table \ref{table:probability}.
The results in Table.~\ref{tab:abl_probability} show that both grayscale and histogram equalization benefit from setting the probability to 1.0. Although \textbf{SA-B5-G3-HE3} does not have the highest average accuracy, we still chose it as our data augmentation combination to simplify the conclusion. The discussion for setting the probability to 1 is left as our future work.

%SA-B5-G3:DataAug44
%SA-B5-Equal3:DataAug46
%SA-B5-G3-Equal3:DataAug45




%SA-B5-G3:DataAug44
%SA-B5-Equal3:DataAug46
%SA-B5-G3-Equal3:DataAug45


\begin{table}[t]
\centering
\small
\caption{Experimental results of histogram equalization and grayscale with probability of 1.0.} 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}l@{ \ }c@{ \ }c@{ \ }c@{ \ }c@{ \ }c@{ \ }c@{}}
    \hline
    % Cut-off frequency                 & LFW   & AgeDB-30 & CA-LFW & CFP-FP & CP-LFW & Avg.  \\ \hline
    Data Aug. & LFW & AgeDB-30 & CA-LFW & CFP-FP & CP-LFW & Avg. \\ \hline
    % {SA-B5-G3} & 95.73 & 78.13    & 80.87  & 85.37  &  79.43 & 83.91 \\ 
    {SA-B5-HE3} & 93.73 & 77.55    & 77.73  & 62.43  & 76.50  & 77.59 \\ 
    {SA-B5-G3-HE3} & \textbf{95.47} & \textbf{77.97}    & \textbf{81.65}  & \textbf{84.89}  & \textbf{79.22}  & \textbf{83.84} \\
    \hline
    \end{tabular}
    }
\label{tab:abl_probability}
\end{table}


==> supplementary_files/SA_ablation_apparance.tex <==
\subsection{Appearance methods}
Following the data augmentation setting of Adaface~\cite{kim2022adaface}, we combine \textbf{low resolution} (LR), \textbf{cropping} (crop), and \textbf{photometric} (Pho) as base augmentation combination (\textbf{SA-B0}) with the same probability of 0.2 in Table.~\ref{table: base and gray scale}. 
We also introduce a stronger base augmentation with probability of 0.5, which we named \textbf{SA-B1}. 
All of our data augmentation experiments base on these two base augmentations.

\subsubsection{Using grayscale or not}
\label{sec:abl_base_grayscale}
To begin, we investigate the impact of applying grayscale during our training stage. 
We have tested various combinations of settings, as shown in Table.~\ref{table: base and gray scale} and Table~\ref{tab:abl_base_and_grayscale}.
Our experimental results demonstrate the significant benefits of using the grayscale method with both SA-B0 and SA-B1.
These results suggest that it is advisable to include grayscale as a standard part of our SA pipeline.

%SA-B1: DataAug100
%SA-B0-G0: DataAug1
%SA-B0-G1: DataAug101
%SA-B1-G1: DataAug2
%SA-B1-G2: DataAug10
\begin{table*}[t]
    \centering
    \caption{Notations and settings for SA about base augmentation and grayscale.}
    \begin{tabular}{l|l|ccccccc}
    \toprule
    Name  & Description & $p^{LR}$  & $p^{Crop}$ & $p^{Pho}$ & $p^{Gray}$   \\ \midrule
    SA-B0 & Original in \cite{kim2022adaface}, base augmentation          & 0.2 & 0.2  & 0.2 & -      \\
    SA-B1 & Stronger base augmentation          & 0.5 & 0.5  & 0.5 & -       \\
    SA-B0-G0 & Add grayscale into SA-B0  & 0.2 & 0.2  & 0.2 & 0.01        \\
    SA-B0-G1 & Add stronger grayscale into SA-B0  & 0.2 & 0.2  & 0.2 & 0.2         \\
    SA-B1-G1 & Add stronger grayscale into SA-B1  & 0.5 & 0.5  & 0.5 & 0.2       \\
    SA-B1-G2 & Add much stronger grayscale into SA-B1  & 0.5 & 0.5  & 0.5 & 0.4        \\
    \bottomrule
    \end{tabular}
    \label{table: base and gray scale}
\end{table*}
\begin{table*}[t]
    \centering
    \caption{Notations and settings for SA about channel shuffle.}
    \begin{tabular}{c|l|ccccccc}
    \toprule
    Name  & Description & $p^{LR}$  & $p^{Crop}$ & $p^{Pho}$ & $p^{Gray}$ & $p^{CS}$  \\ \midrule
    SA-B0-CS0 & Add Channel shuffle into SA-B0  & 0.2 & 0.2  & 0.2 & - &  0.01     \\
    SA-B1-CS1 & Add Channel shuffle into SA-B1  & 0.5 & 0.5  & 0.5 & - &  0.2      \\
    SA-B2-CS1 & Add Channel shuffle into SA-B1-G1  & 0.5 & 0.5  & 0.5 & 0.2 &  0.2  \\
    \bottomrule
    \end{tabular}
    \label{table:channel-shuffle}
\end{table*}
\begin{table*}[t]
    \centering
    \caption{Notations and settings for SA about Gaussian noise and Gaussian blur.}
    \begin{tabular}{l|l|ccccccc}
    \toprule
    Name  & Description & $p^{LR}$  & $p^{Crop}$ & $p^{Pho}$ & $p^{Gray}$  & $p^{GB}$  & $p^{GN}$  \\ \midrule
    SA-B2-GB0 & Add GN into SA-B1-G1  & 0.5 & 0.5  & 0.5 & 0.2    & 0.2   &  -  \\
    SA-B2-GN0 & Add GN into SA-B1-G1  & 0.5 & 0.5  & 0.5 & 0.2   & -   &  0.2  \\
    SA-B2-GB0-GN0 & Add GN into SA-B1-G1  & 0.5 & 0.5  & 0.5 & 0.2    & 0.2   &  0.2  \\
    SA-B3-GB1-GN1 & Add GN into SA-B1-G2  & 0.5 & 0.5  & 0.5 & 0.4   & 0.4   &  0.4  \\
    
    \bottomrule
    \end{tabular}
    \label{table:gaussian-blur-and-gaussian-noise}
\end{table*}
\begin{table}[t]
    \centering
    \caption{Notations and settings for geometry methods. }
    \begin{tabular}{c|l|ccccccc}
    \toprule
    Name  & Base & $p^{Per}$ & $p^{Aff}$  \\ \midrule
    SA-B1-Per0 & SA-B1          & 0.2 & -  \\
    SA-B1-Aff0 & SA-B1          & - & 0.2   \\
    SA-B4-Per1 & SA-B3-GB1-GN1  & 0.4 & -  \\
    SA-B4-Aff1 & SA-B3-GB1-GN1  & - & 0.4  \\
    
    \bottomrule
    \end{tabular}
    \label{table:geometry}
\end{table}

\begin{table}[t]
\centering
\small
\caption{Ablation study for  histogram equalization and autocontrast.} 
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}l@{ \ }c@{ \ }c@{ \ }c@{ \ }c@{ \ }c@{ \ }c@{}}
    \hline
    % Cut-off frequency                 & LFW   & AgeDB-30 & CA-LFW & CFP-FP & CP-LFW & Avg.  \\ \hline
    Data Aug.                  & LFW & AgeDB-30 & CA-LFW & CFP-FP & CP-LFW & Avg. \\ \hline
    {SA-B0-HE0}                        & 89.37 & 70.03    & 73.45  & 77.66  &  70.13 & 76.13 \\ 
    {SA-B0-HE1}                        & 90.77 & 72.85    & 73.93  & 79.17  & 70.68  & 77.48 \\ 
    {SA-B1-HE1}                        & 90.63 & 72.63    & 75.93  & 79.64  & 71.90  & 78.15 \\
    {SA-B1-HE2}                        & 91.00 & 74.10    & 76.10  & 79.93  & 72.17  & 78.66 \\
    {SA-B0-HE3}                        & \textbf{92.40} & 74.37    & 75.58  & 80.64  & 72.33  & 79.07 \\
    {SA-B1-HE3}                        & 92.17 & \textbf{75.07}    & \textbf{77.08}  & \textbf{81.46}  & \textbf{74.23} & \textbf{80.00} \\

    {SA-B0-AC0}                        & 88.33 & 67.46    & 62.66  & 76.51  &  68.37 & 74.67 \\ 
    {SA-B0-AC1}                        & 88.70 & 70.22    & 72.65  & 77.09  & 69.88  & 75.71 \\ 
    {SA-B1-AC1}                        & 88.83 & 71.77    & 73.95  & 78.14  & 69.48  & 76.44 \\
    {SA-B1-AC2}                        & 89.48 & 71.60    & 73.02  & 78.29  & 70.78  & 76.63 \\
    {SA-B0-AC3}                        & 89.80 & 68.90    & 72.32  & 77.59  & 69.43  & 75.61 \\
    {SA-B1-AC3}                        & 89.35 & 72.63    & 73.87  & 79.11  & 71.28  & 77.25 \\
    \hline
    \end{tabular}
    }
\label{tab:abl_equalization_and_autocontrast}
\end{table}

\begin{table}[t]
    \centering
    \caption{Notations and settings for histogram equalization and autocontrast.}
    \begin{tabular}{l|l|ccccccc}
    \toprule
    Name  & Base & $p^{Equal}$ & $p^{AC}$  \\ \midrule
    SA-B0-HE0 & SA-B0          & 0.05 & -  \\
    SA-B0-HE1 & SA-B0          & 0.2 & -  \\
    SA-B1-HE1 & SA-B0          & 0.2 & -  \\
    SA-B1-HE2 & SA-B0          & 0.4 & -  \\
    SA-B0-HE3 & SA-B0          & 1.0 & -  \\
    SA-B1-HE3 & SA-B0          & 1.0 & -  \\
    SA-B0-AC0 & SA-B0          & - & 0.05  \\
    SA-B0-AC1 & SA-B0          & - & 0.2  \\
    SA-B1-AC1 & SA-B0          & - & 0.2  \\
    SA-B1-AC2 & SA-B0          & - & 0.4  \\
    SA-B0-AC3 & SA-B0          & - & 1.0  \\
    SA-B1-AC3 & SA-B0          & - & 1.0  \\
    
    \bottomrule
    \end{tabular}
    \label{table:equalization_and_autocontrast}
\end{table}
\begin{table}[t]
    \centering
    \caption{Notations and settings for histogram equalization and grayscale with probability of 1.0.}
    \begin{tabular}{l|l|ccccccc}
    \toprule
    Name  & Base & $p^{Gray}$ & $p^{Equal}$  \\ \midrule
    % SA-B5-G3 & SA-B4-Per1          & 1.0 & -  \\
    SA-B5-HE3 & SA-B4-Per1          & - & 1.0  \\
    SA-B5-G3-HE3 & SA-B4-Per1          & 1.0 & 1.0  \\
    \bottomrule
    \end{tabular}
    \label{table:probability}
\end{table}
\begin{table}[t]
    \centering
    \caption{Notations and settings for order. ``T" denotes true, and ``F" denotes false.}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|l|cccc}
    \toprule
    Name  & Base & $Gray_{first}$ & $Gray_{last}$ & $HE_{first}$ & $HE_{last}$ \\ \midrule
    SA-B6-O1 & SA-B5-G3-HE3  & T & F & F & T  \\
    SA-B6-O2 & SA-B5-G3-HE3  & F & T & F & T  \\
    SA-B6-O3 & SA-B5-G3-HE3  & F & T & T & F \\
    SA-B6-O4 & SA-B5-G3-HE3  & T & T & T & F \\
    SA-B6-O5 & SA-B5-G3-HE3  & F & T & T & T \\
    SA-B6-O6 & SA-B5-G3-HE3  & T & F & T & T  \\
    SA-B6-O7 & SA-B5-G3-HE3  & T & T & F & T \\
    SA-B6-O8 & SA-B5-G3-HE3  & T & T & T & T \\
    
    
    \bottomrule
    \end{tabular}
    }
    \label{table:order}
\end{table}

%SA-B1: DataAug100
%SA-B0-G0: DataAug1
%SA-B0-G1: DataAug101
%SA-B1-G1: DataAug2
%SA-B1-G2: DataAug10

\begin{table}[t]
\centering
\small
\caption{Ablation study for base augmentation and grayscale.} 
    \begin{tabular}{@{}l@{ \ }c@{ \ }c@{ \ }c@{ \ }c@{ \ }c@{ \ }c@{}}
    \hline
    Data Aug. & LFW & AgeDB-30 & CA-LFW & CFP-FP & CP-LFW & Avg. \\ \hline
    {SA-B0}    & 88.43 & 67.27    & 71.52  & 76.57  &  69.45 & 74.65 \\ 
    {SA-B1}    & 88.77 & 69.40    & 72.05  & 76.50  & 70.50  & 75.44 \\ 
    {SA-B0-G0} & 88.88 & 71.30    & 73.15  & 78.10  & 70.85  & 76.45 \\ 
    {SA-B0-G1} & 90.33 & 72.10    & 75.43  & 79.53 & 72.05  & 77.89 \\  
    {SA-B1-G1} & 91.55 & \textbf{76.72}    & 77.12  & \textbf{81.27}  & 73.05  & \textbf{79.94} \\ 
    {SA-B1-G2} & \textbf{91.83} & 75.23    & \textbf{77.38}  & 81.09  & \textbf{73.67}  & 79.84 \\ 
    \hline
    \end{tabular}
\label{tab:abl_base_and_grayscale}
\end{table}

\subsubsection{Using channel shuffle or not}
\label{sec:abl_channel_shuffle}
Building on our previous findings, we further investigate the impact of channel shuffle as a data augmentation method. 
In addition to \textbf{SA-B0} and \textbf{SA-B1}, we also test \textbf{SA-B1-G1} as a new base augmentation, which we denote as \textbf{SA-B2}. 
The combination settings for channel shuffle are recorded in Table~\ref{table:channel-shuffle}, and the results are presented in Table~\ref{tab:abl_channel_shuffle}. 
Although channel shuffle showed promising results when applied to \textbf{SA-B0} and \textbf{SA-B1}, it had a negative impact on the performance of \textbf{SA-B1-G1}. 
Given the importance of maintaining a stable and reliable data augmentation pipeline, we decided to remove channel shuffle from our list of SA methods.
% In order to ensure a stable and reliable data augmentation pipeline, it is important to remove any potential threats to performance. 
% Therefore, we have decided to remove channel shuffle from our list of SA.
 
%SA-B0-CS0: DataAug13
%SA-B1-CS1: DataAug14
%SA-B2-CS1: DataAug15



%SA-B0-CS0: DataAug13
%SA-B1-CS1: DataAug14
%SA-B2-CS1: DataAug15

\begin{table}[t]
\centering
\small
\caption{Ablation study for channel shuffle.} 
    \begin{tabular}{@{}l@{ \ }c@{ \ }c@{ \ }c@{ \ }c@{ \ }c@{ \ }c@{}}
    \hline
    % Cut-off frequency                 & LFW   & AgeDB-30 & CA-LFW & CFP-FP & CP-LFW & Avg.  \\ \hline
    Data Aug.                  & LFW & AgeDB-30 & CA-LFW & CFP-FP & CP-LFW & Avg. \\ \hline
    {SA-B0-CS0}                        & 87.97 & 70.13    & 72.82  & 77.43  &  68.87 & 75.44 \\ 
    {SA-B1-CS1}                        & 89.37 & 73.00    & 75.72  & 78.61  & 71.43  & 77.63 \\ 
    {SA-B2-CS1}                        & 91.87 & 75.45    & 77.47  & 81.09  & 73.52  & 79.88 \\
    % $D_{0}\sim U(S)$ & 95.72 & 79.32    & 81.57  & 84.97  & 80.33  & 84.38 \\ 
    \hline
    % $D_{0}\sim U(15, 60)$             & 95.77 & 78.83    & 81.27  & 85.11  & 79.57  & 84.11 \\ \hline 
    \end{tabular}
\label{tab:abl_channel_shuffle}
\end{table}



\subsubsection{Gaussian Noise and Gaussian Blur}
\label{sec:abl_gaussian_blur_and_gaussian_noise}
Based on the results from section \ref{sec:abl_base_grayscale}, we expand our SA pipeline to include Gaussian blur and Gaussian noise. 
% Our new base augmentation is \textbf{SA-B1-G1} and we denote as \textbf{SA-B2}.
We conduct the following experiment upon \textbf{SA-B2}.
We have tested various combinations of Gaussian blur and Gaussian noise, and the experiment settings are presented in Table~\ref{table:gaussian-blur-and-gaussian-noise}.
The results are shown in Table~\ref{tab:abl_gaussian_blur_and_gaussian_noise}.
Although Gaussian blur had a more significant impact when applied individually than Gaussian noise, using these two techniques jointly in the \textbf{SA-B1-G1} pipeline still showed a considerable improvement over using Gaussian blur alone.
Thus, we decided to pair Gaussian blur and Gaussian noise and add them to the SA pipeline with equal probability.
In addition, we get better performance when using \textbf{SA-B1-G2} with $p^{GN}=0.4$ and $p^{GB}=0.4$ (\textbf{SA-B3-GB1-GN1}).
 
% We selected \textbf{SA-B1-G1} as the new base augmentation. 
% The experiment settings for these two techniques are presented in Table.~\ref{table:gaussian-blur-and-gaussian-noise}, and the results are shown in Table.~\ref{tab:abl_gaussian_blur_and_gaussian_noise}. 
% While Gaussian blur had a more pronounced impact when applied individually, in contrast to Gaussian noise, these two techniques jointly added to \textbf{SA-B1-G1} still showed a significant improvement over using Gaussian blur individually. 
% Therefore, we have decided to pair these two augmentations and add them to the SA pipeline with the same probability.



%SA-B2-GB0: DataAug6
%SA-B2-GN0: DataAug12
%SA-B2-GB0-GN0: DataAug7
%SA-B3-GB1-GN1: DataAug102



%SA-B2-GB0: DataAug6
%SA-B2-GN0: DataAug12
%SA-B2-GB0-GN0: DataAug7
%SA-B3-GB1-GN1: DataAug102

\begin{table}[t]
\centering
\footnotesize
\caption{Ablation study for Gaussian noise and Gaussian blur.} 
    \begin{tabular}{@{}l@{ \ }c@{ \ }c@{ \ }c@{ \ }c@{ \ }c@{ \ }c@{}}
    \hline
    % Cut-off frequency                 & LFW   & AgeDB-30 & CA-LFW & CFP-FP & CP-LFW & Avg.  \\ \hline
    Data Aug. & LFW & AgeDB-30 & CA-LFW & CFP-FP & CP-LFW & Avg. \\ \hline
    {SA-B2-GB0} & 91.97 & 76.02    & 78.68  & 80.77  &  74.05 & 80.30 \\ 
    {SA-B2-GN0} & 91.45 & 74.85    & 76.75  & 81.86  & 72.67  & 79.51 \\ 
    {SA-B2-GB0-GN0} & 92.10 & 76.63    & 78.17  & 81.79  & 73.17  & 80.37 \\ 
    {SA-B3-GB1-GN1} & \textbf{94.00} & \textbf{77.92}    & \textbf{79.68}  & \textbf{82.39} & \textbf{77.05}  & \textbf{82.21} \\  
    
    % $D_{0}\sim U(S)$ & 95.72 & 79.32    & 81.57  & 84.97  & 80.33  & 84.38 \\ 
    \hline
    % $D_{0}\sim U(15, 60)$             & 95.77 & 78.83    & 81.27  & 85.11  & 79.57  & 84.11 \\ \hline 
    \end{tabular}
    \label{tab:abl_gaussian_blur_and_gaussian_noise}
\end{table}

==> supplementary_files/SA_ablation_geometry.tex <==
\subsection{Geometry methods}
\label{sec:abl_geometry}
Real-world images present not only appearance challenges but also distortion challenges. To enhance the robustness of our model when facing real-world images, we incorporated mimic distortion as a data augmentation method. To prevent over-distortion, we select either random perspective or random affine based on which method provides the greatest performance boost.

We select \textbf{SA-B1} from Section~\ref{sec:abl_base_grayscale} and \textbf{SA-B3-GB1-GN1} from Section~\ref{sec:abl_gaussian_blur_and_gaussian_noise} as the new base augmentations, denoted as \textbf{SA-B4}. Table~\ref{table:geometry} shows the experiment settings, and the results are presented in Table~\ref{tab:abl_geometry}. Regardless of the base augmentation, the random perspective consistently outperformed the random affine. Therefore, we have decided to include the random perspective in our data augmentation pipeline with a probability of 0.4.

%SA-B1-Per0: DataAug23
%SA-B1-Aff0: DataAug8
%SA-B4-Per1: DataAug21
%SA-B4-Aff1: DataAug11



%SA-B1-Per0: DataAug23
%SA-B1-Aff0: DataAug8
%SA-B4-Per1: DataAug21
%SA-B4-Aff1: DataAug11

\begin{table}[t]
\centering
\small
\caption{Ablation study for geometry methods.} 
    \begin{tabular}{@{}l@{ \ }c@{ \ }c@{ \ }c@{ \ }c@{ \ }c@{ \ }c@{}}
    \hline
    % Cut-off frequency                 & LFW   & AgeDB-30 & CA-LFW & CFP-FP & CP-LFW & Avg.  \\ \hline
    Data Aug.                  & LFW & AgeDB-30 & CA-LFW & CFP-FP & CP-LFW & Avg. \\ \hline
    {SA-B1-Per0}                        & 88.97 & 67.22    & 72.15  & 79.17  &  71.27 & 75.75 \\ 
    {SA-B1-Aff0}                        & 89.47 & 67.88    & 71.70  & 77.80  & 70.30  & 75.43 \\ 
    {SA-B4-Per1}                        & \textbf{94.00} & \textbf{77.75}    & \textbf{79.97}  & \textbf{84.17}  & \textbf{78.38}  & \textbf{82.85} \\
    {SA-B4-Aff1}                        & 93.98 & 77.15    & 77.63  & 79.81  & 74.13  & 80.54 \\
    % $D_{0}\sim U(S)$ & 95.72 & 79.32    & 81.57  & 84.97  & 80.33  & 84.38 \\ 
    \hline
    % $D_{0}\sim U(15, 60)$             & 95.77 & 78.83    & 81.27  & 85.11  & 79.57  & 84.11 \\ \hline 
    \end{tabular}
\label{tab:abl_geometry}
\end{table}



==> supplementary_files/SA_ablation_order_of_data_augmentation.tex <==
\subsection{Order of SA}
\label{sec:abl_order}
After finalizing our SA list, \textbf{SA-B5-G3-HE3}, we consider the order of applying SA to further optimize our model performance. 
We focus on the order of grayscale and histogram equalization in combination with other SA methods. 
Moreover, we explore how many times we can apply grayscale or histogram equalization. Our initial implementation applied both grayscale and histogram equalization before other data augmentation methods. 
We test different orders of applying SA, as shown in Table.~\ref{tab:abl_order}. 
We use the notation $Gray_{first}$ to indicate applying grayscale first, and $HE_{first}$ to indicate applying histogram equalization first. 
If both adopted simultaneously, we apply grayscale first followed by histogram equalization. 
$Gray_{last}$ and $HE_{last}$ denote applying at the last.
We choose \textbf{SA-B6-O4} as our final proposed SA based on the average accuracy.
% Our proposed SA, \textbf{SA-B6-O4}, achieves the highest average accuracy.
%SA-B6-O1: DataAug48
%SA-B6-O2: DataAug49
%SA-B6-O3: DataAug50
%SA-B6-O4: DataAug51
%SA-B6-O5: DataAug52
%SA-B6-O6: DataAug53
%SA-B6-O7: DataAug54
%SA-B6-O8: DataAug55



%SA-B6-O1: DataAug48
%SA-B6-O2: DataAug49
%SA-B6-O3: DataAug50
%SA-B6-O4: DataAug51
%SA-B6-O5: DataAug52
%SA-B6-O6: DataAug53
%SA-B6-O7: DataAug54
%SA-B6-O8: DataAug55

\begin{table}[t]
\centering
\small
\caption{Ablation study for SA order.} 
    \begin{tabular}{@{}l@{ \ }c@{ \ }c@{ \ }c@{ \ }c@{ \ }c@{ \ }c@{}}
    \hline
    % Cut-off frequency                 & LFW   & AgeDB-30 & CA-LFW & CFP-FP & CP-LFW & Avg.  \\ \hline
    Data Aug.                  & LFW & AgeDB-30 & CA-LFW & CFP-FP & CP-LFW & Avg. \\ \hline
    {SA-B6-O1}                        & 95.35 & 77.57    & 81.33  & 84.19  &  78.63 & 83.41 \\ 
    {SA-B6-O2}                        & 95.57 & 77.90    & \textbf{81.60}  & 84.76  & 79.12  & 83.79 \\ 
    {SA-B6-O3}                        & 95.62 &  77.62  & 80.92  & \textbf{85.27}  & \textbf{79.67}  & 83.82 \\
    {SA-B6-O4}                        & 95.32 & 78.37    & 81.37  & 85.21  & 79.53  & \textbf{83.96} \\
    {SA-B6-O5}                        & 95.15 & 78.48    & 81.45  & 85.01  & 79.22  & 83.86 \\
    {SA-B6-O6}                        & 91.27 & 74.87    & 76.80  & 80.03  & 73.55  & 79.30 \\
    {SA-B6-O7}                        & 95.27 & \textbf{79.28}    & 81.43  & 84.50  & 79.03  & 83.90 \\
    {SA-B6-O8}                        & \textbf{95.72} & 78.73    & 81.15  & 84.57  & 79.42  & 83.92 \\
    \hline
    % $D_{0}\sim U(15, 60)$             & 95.77 & 78.83    & 81.27  & 85.11  & 79.57  & 84.11 \\ \hline 
    \end{tabular}
\label{tab:abl_order}
\end{table}

==> supplementary_files/SA_implementation_visualization.tex <==
\subsection{SA implementation}
There are various types of data augmentation in visual-related task~\cite{shorten2019data_augmentation_survey, mumuni2022data_augmentation_comprehensive_survey}.
In order to maintain focus and facilitate implementation, our selection of candidate methods and probabilities is restricted to the following items as Table.~\ref{tab:data_augmentation_list}.
% Noticed we Additionally, the notation following each item represents its adoption probability.
% The Figure.~\cite{visualization of data augmentation} shows the effect of these data augmentation.

\begin{table*}[t]
\centering
\caption{The details of data augmentation. $p^*$ denote the probability of adopting data augmentation.}
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{|c|l|l|l|}
\hline
& Method & Source and hyperparameter & \tabincell{l}{Notation of \\ probability} \\ \hline
\multirow{9}{*}{Appearance} & Crop & Default in Adaface~\cite{kim2022adaface} & $p^{Crop}$ \\ \cline{2-4}
                            & Low Resolution & Default in Adaface~\cite{kim2022adaface} & $p^{LR}$ \\ \cline{2-4}
                            & Photometric & Default in Adaface~\cite{kim2022adaface} & $p^{Pho}$ \\ \cline{2-4}
                            & Grayscale & Torchvision~\cite{torchvision2016} built-in, remains 3 channels & $p^{Gray}$ \\ \cline{2-4}
                            & Gaussian Noise & skimage~\cite{van2014skimage} built-in, random\_noise(mode="gaussian") & $p^{GN}$ \\ \cline{2-4}
                            & Gaussian Blur & Torchvision~\cite{torchvision2016} built-in, kernel size = (7, 7) & $p^{GB}$ \\ \cline{2-4}
                            & Channel Shuffle & Randomize the order of RGB channels & $p^{CS}$ \\ \cline{2-4}
                            & Histogram Equalization & Torchvision~\cite{torchvision2016} built-in & $p^{HE}$ \\ \cline{2-4}
                            & Autocontrast & Torchvision~\cite{torchvision2016} built-in & $p^{AC}$ \\ \hline
\multirow{2}{*}{Geometry}   & Random Affine & \tabincell{l}{Torchvision~\cite{torchvision2016} built-in, \\ degrees=(-30,30), translate=(0, 0.5), scale=(0.4, 0.5), shear=(0,0)} & $p^{RA}$ \\ \cline{2-4}
                            & Random Perspective & \tabincell{l}{Torchvision~\cite{torchvision2016} built-in,\\ distortion\_scale=np.random.uniform(0.0, 0.5)} & $p^{RP}$ \\ \hline
\end{tabular}
\label{tab:data_augmentation_list}
\end{table*}

% \begin{table*}[t]
% \centering
% \caption{\label{tab:data_augmentation_list}
% The details of applied data augmentation}
% \begin{tabular}{@{}|c|c|c|c|@{}}
% \toprule
% \multicolumn{1}{|l|}{}      & Name                                                              & Implementation and Hyperparameter                                                                                          & Notation of probabilty \\ \midrule
% \multirow{9}{*}{Appearance} & Crop                                                              & Default in Adaface~\cite{kim2022adaface}                                                                                                         &          $p^{Crop}$              \\ \cmidrule(l){2-4} 
%                             & \begin{tabular}[c]{@{}c@{}}Low Resolution\\ (LR)\end{tabular}     & Default in Adaface~\cite{kim2022adaface}                                                                                                         &         $p^{LR}$               \\ \cmidrule(l){2-4} 
%                             &   
%                             \begin{tabular}[c]{@{}c@{}}Photometric\\ (Pho)\end{tabular} & Default in Adaface~\cite{kim2022adaface}                                                                                                         &     $p^{Photometric}$                   \\ \cmidrule(l){2-4} 
%                             & \begin{tabular}[c]{@{}c@{}}Grayscale\\ (Gray)\end{tabular}                                                        & Torchvision~\cite{torchvision2016} built-in, remains 3 channels                                                                                 & $p^{Grayscale}$                       \\ \cmidrule(l){2-4} 
%                             & \begin{tabular}[c]{@{}c@{}}Gaussian Noise\\ (GN)\end{tabular}     & 
%                             \begin{tabular}[c]{@{}c@{}}Use skimage~\cite{van2014skimage} built-in \\ skimage.util.random\_noise(mode="gaussian")\end{tabular}                                                         &  $p^{GN}$                      \\ \cmidrule(l){2-4} 
%                             & \begin{tabular}[c]{@{}c@{}}Gaussian Blur\\ (GB)\end{tabular}      & Torchvision~\cite{torchvision2016} built-in, kernel size = (7,7)                                                                                           &       $^{GB}$                 \\ \cmidrule(l){2-4} 
%                             & \begin{tabular}[c]{@{}c@{}}Channel Shuffle\\ (CS)\end{tabular}    & Ramdomize the order of RGB channels                                                                                            &           $p^{CS}$             \\ \cmidrule(l){2-4} 
%                             & Equalize                                                          & Torchvision~\cite{torchvision2016} built-in                                                                                                     &   $p^{Equalize}$                     \\ \cmidrule(l){2-4} 
%                             & \begin{tabular}[c]{@{}c@{}}Auto Contrast\\ (AC)\end{tabular}      & Torchvision~\cite{torchvision2016} built-in                                                                                                     &         $p^{AC}$              \\ \midrule
% \multirow{2}{*}{Geometry}   & \begin{tabular}[c]{@{}c@{}}Random Affine\\ (Aff)\end{tabular}      & \begin{tabular}[c]{@{}c@{}}Torchvision~\cite{torchvision2016} built-in,\\ degrees=(-30,30), translate=(0, 0.5), scale=(0.4, 0.5), shear=(0,0)\end{tabular} &          $p^{RA}$              \\ \cmidrule(l){2-4} 
%                             & \begin{tabular}[c]{@{}c@{}}Random Perspective\\ (Per)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Torchvision~\cite{torchvision2016} built-in,\\ distortion\_scale=np.random.uniform(0.0, 0.5)\end{tabular}                       &  $p^{RP}$                      \\ \bottomrule
% \end{tabular}
% \end{table*}
